ID-like Prompt Learning for Few-Shot Out-of-Distribution Detection

Out-of-distribution (OOD) detection methods often exploit auxiliary outliers to train model identifying OOD samples, especially discovering challenging outliers from auxiliary outliers dataset to improve OOD detection. However, they may still face limitations in effectively distinguishing between the most challenging OOD samples that are much like in-distribution (ID) data, i.e., \idlike samples. To this end, we propose a novel OOD detection framework that discovers \idlike outliers using CLIP \cite{DBLP:conf/icml/RadfordKHRGASAM21} from the vicinity space of the ID samples, thus helping to identify these most challenging OOD samples. Then a prompt learning framework is proposed that utilizes the identified \idlike outliers to further leverage the capabilities of CLIP for OOD detection. Benefiting from the powerful CLIP, we only need a small number of ID samples to learn the prompts of the model without exposing other auxiliary outlier datasets. By focusing on the most challenging \idlike OOD samples and elegantly exploiting the capabilities of CLIP, our method achieves superior few-shot learning performance on various real-world image datasets (e.g., in 4-shot OOD detection on the ImageNet-1k dataset, our method reduces the average FPR95 by 12.16\% and improves the average AUROC by 2.76\%, compared to state-of-the-art methods). Code is available at https://github.com/ycfate/ID-like.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/t3.tex <==
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{-10pt}
\begin{table*}[t]
\caption{OOD detection performance for ImageNet-100 as ID.}
\label{result_100}
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{\textwidth}{
p{2.7cm}
c@{\hspace{3pt}}c
c@{\hspace{3pt}}c
c@{\hspace{3pt}}c
c@{\hspace{3pt}}c
c@{\hspace{3pt}}c
}

\hline
~ & \multicolumn{10}{c}{OOD Dataset}\\
Method 
& \multicolumn{2}{c}{iNaturalist} 
& \multicolumn{2}{c}{SUN} 
& \multicolumn{2}{c}{Places} 
& \multicolumn{2}{c}{Texture} 
& \multicolumn{2}{c}{Average}\\
\cmidrule(r){2-3}  \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11}

~ 
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}\\

\hline
~ & \multicolumn{10}{c}{Full/Sub Data Fine-tune}\\
Fort/MSP \citep{DBLP:conf/nips/FortRL21}
            & 49.48 & 93.72 & 38.56 & 93.16 & 41.30 & 91.53 & 38.16 & 93.53 & 41.87 & 92.98 \\
Energy \citep{DBLP:conf/nips/LiuWOL20}
            & 20.95 & 95.94 & 18.42 & 94.77 & 22.35 & 93.08 & 15.36 & 96.19 & 19.27 & 94.99 \\
ODIN \citep{DBLP:conf/iclr/LiangLS18}
            & 7.32 & 98.09 & 29.05 & 92.63 & 32.58 & 92.60 & 15.50 & 96.58 & 21.11 & 94.98 \\
GradNorm \citep{DBLP:conf/nips/HuangGL21}
            & 28.72 & 91.14 & 54.41 & 73.08 & 43.02 & 81.13 & 28.28 & 91.29 & 38.61 & 84.16 \\
ViM \citep{DBLP:conf/cvpr/Wang0F022}
            & 13.75 & 96.67 & 31.68 & 93.31 & 39.61 & 88.95 & 26.94 & 94.13 & 28.00 & 93.27 \\
KNN \citep{DBLP:conf/icml/SunM0L22}
            & 6.77 & 98.21 & 26.72 & 92.87 & 23.13 & 92.81 & 15.02 & 96.73 & 17.91 & 95.16 \\
VOS \citep{DBLP:conf/iclr/DuWCL22}
            & 8.05 & 98.03 & 29.54 & 92.91 & 29.54 & 92.91 & 13.79 & 97.28 & 19.16 & 95.69 \\
VOS+        & 8.44 & 98.00 & 17.58 & 96.69 & 17.46 & 95.95 & 16.85 & 96.43 & 15.08 & 96.77 \\
NPOS \citep{DBLP:conf/iclr/TaoDZ023}
            & 0.70 & 99.14 &  9.22 & 98.48 &  5.12 & 98.86 &  8.01 & 98.47 &  5.76 & 98.74 \\
\hline
~ & \multicolumn{10}{c}{Zero-shot}\\
MCM \citep{DBLP:conf/nips/MingCGSL022}
            & 15.23 & 97.30 & 25.05 & 95.95 & 24.91 & 95.66 & 33.68 & 94.11 & 24.72 & 95.76 \\
\hline
~ & \multicolumn{10}{c}{One-shot}\\
Ours        & 10.82 & 97.84 & 41.94 & 91.43 & 26.60 & 95.07 & 20.41 & 96.16 & 24.94 & 95.12 \\
\hline
~ & \multicolumn{10}{c}{Four-shot}\\
Ours        &  1.62 & 99.60 & 29.53 & 93.70 & 20.81 & 96.05 & 13.55 & 97.30 & 16.38 & 96.66 \\
\hline
\end{tabularx}
\end{table*}


==> tables/t4.tex <==
% \setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{-10pt}
\begin{table*}[t]
\caption{OOD detection performance for ImageNet-100 as ID, and trained on our data.}
\label{result_100_our_data}
\renewcommand{\arraystretch}{1.2}
\begin{tabularx}{\textwidth}{
p{2.7cm}
c@{\hspace{3pt}}c
c@{\hspace{3pt}}c
c@{\hspace{3pt}}c
c@{\hspace{3pt}}c
c@{\hspace{3pt}}c
}

\hline
~ & \multicolumn{10}{c}{OOD Dataset}\\
Method 
& \multicolumn{2}{c}{iNaturalist} 
& \multicolumn{2}{c}{SUN} 
& \multicolumn{2}{c}{Places} 
& \multicolumn{2}{c}{Texture} 
& \multicolumn{2}{c}{Average}\\
\cmidrule(r){2-3}  \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11}

~ 
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}\\

\hline
~ & \multicolumn{10}{c}{One-shot}\\
MSP \citep{DBLP:conf/iclr/HendrycksG17}
            & 98.56 & 32.83 & 96.63 & 50.31 & 94.30 & 53.56 & 94.63 & 34.09 & 96.03 & 42.70 \\
Fort/MSP \citep{DBLP:conf/nips/FortRL21}
            & 63.89 & 85.17 & 73.65 & 71.95 & 73.07 & 78.02 & 76.47 & 77.18 & 71.77 & 78.08\\
Energy \citep{DBLP:conf/nips/LiuWOL20}
            & 97.13 & 47.39 & 87.83 & 60.16 & 88.75 & 59.82 & 75.85 & 69.05 & 87.39 & 59.11 \\
Mahalanobis \citep{DBLP:conf/nips/LeeLLS18}
            & 99.78 & 52.41 & 99.51 & 56.55 & 98.58 & 61.50 & 99.61 & 46.61 & 99.37 & 54.27\\
Ours        & 10.82 & 97.84 & 41.94 & 91.43 & 26.60 & 95.07 & 20.41 & 96.16 & 24.94 & 95.12 \\
\hline
~ & \multicolumn{10}{c}{Four-shot}\\
MSP \citep{DBLP:conf/iclr/HendrycksG17}
            & 94.47 & 54.12 & 96.29 & 45.68 & 96.42 & 44.41 & 86.21 & 48.37 & 93.35 & 48.14 \\
Fort/MSP \citep{DBLP:conf/nips/FortRL21}
            & 37.14 & 93.47 & 57.04 & 85.79 & 53.49 & 88.59 & 68.60 & 83.16 & 54.07 & 87.75\\
Energy \citep{DBLP:conf/nips/LiuWOL20}
            & 89.27 & 62.00 & 89.01 & 60.15 & 88.66 & 59.24 & 69.34 & 75.58 & 84.07 & 64.24 \\
Mahalanobis \citep{DBLP:conf/nips/LeeLLS18}
            & 99.42 & 60.78 & 99.28 & 59.46 & 97.91 & 65.83 & 99.27 & 56.02 & 98.97 & 60.52\\
Ours        & 10.82 & 97.84 & 41.94 & 91.43 & 26.60 & 95.07 & 20.41 & 96.16 & 24.94 & 95.12 \\
\hline
\end{tabularx}
\end{table*}


==> tables/t_.tex <==
\setlength{\abovecaptionskip}{3pt}
\setlength{\belowcaptionskip}{-10pt}
\begin{table*}[t]
\caption{OOD detection performance for ImageNet-1k \citep{DBLP:conf/cvpr/DengDSLL009} as ID.}
\label{result_1k_back}
\renewcommand{\arraystretch}{1.0}
\begin{tabularx}{\textwidth}{
p{2.7cm}
c@{\hspace{4pt}}c
c@{\hspace{4pt}}c
c@{\hspace{4pt}}c
c@{\hspace{4pt}}c
c@{\hspace{4pt}}c
}

\hline
~ & \multicolumn{10}{c}{OOD Dataset}\\
Method 
& \multicolumn{2}{c}{iNaturalist} 
& \multicolumn{2}{c}{SUN} 
& \multicolumn{2}{c}{Places} 
& \multicolumn{2}{c}{Texture} 
& \multicolumn{2}{c}{Average}\\
\cmidrule(r){2-3}  \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11}

~ 
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont FPR95↓}
& \multicolumn{1}{c}{\fontsize{8}{14}\selectfont AUROC↑}\\

\hline
~ & \multicolumn{10}{c}{Full/Sub Data Fine-tune}\\
MSP \citep{DBLP:conf/iclr/HendrycksG17}
            & 40.89 & 88.63 & 65.81 & 81.24 & 67.90 & 80.14 & 64.96 & 78.16 & 59.89 & 82.04 \\
Fort/MSP \citep{DBLP:conf/nips/FortRL21}
            & 54.05 & 87.43 & 73.37 & 78.03 & 72.98 & 78.03 & 68.85 & 79.06 & 67.31 & 80.64 \\
Energy \citep{DBLP:conf/nips/LiuWOL20}
            & 29.75 & 94.68 & 53.18 & 87.33 & 56.40 & 85.60 & 51.35 & 88.00 & 47.67 & 88.90 \\
ODIN \citep{DBLP:conf/iclr/LiangLS18}
            & 30.22 & 94.65 & 54.04 & 87.17 & 55.06 & 85.54 & 51.67 & 87.85 & 47.75 & 88.80 \\
GradNorm \citep{DBLP:conf/nips/HuangGL21}
            & 81.50 & 72.56 & 82.00 & 72.86 & 80.41 & 73.70 & 79.36 & 70.26 & 80.82 & 72.35 \\
ViM \citep{DBLP:conf/cvpr/Wang0F022}
            & 32.19 & 93.16 & 54.01 & 87.19 & 60.67 & 83.75 & 53.94 & 87.18 & 50.20 & 87.82 \\
KNN \citep{DBLP:conf/icml/SunM0L22}
            & 29.17 & 94.52 & 35.62 & 92.67 & 39.61 & 91.02 & 64.35 & 85.67 & 42.19 & 90.97 \\
VOS \citep{DBLP:conf/iclr/DuWCL22}
            & 31.65 & 94.53 & 43.03 & 91.92 & 41.62 & 90.23 & 56.67 & 86.74 & 43.24 & 90.86 \\
VOS+        & 28.99 & 94.62 & 36.88 & 92.57 & 38.39 & 91.23 & 61.02 & 86.33 & 41.32 & 91.19 \\
NPOS \citep{DBLP:conf/iclr/TaoDZ023}
            & 16.58 & 96.19 & 43.77 & 90.44 & 45.27 & 89.44 & 46.12 & 88.80 & 37.93 & 91.22 \\
\hline
~ & \multicolumn{10}{c}{Zero-shot}\\
MCM \citep{DBLP:conf/nips/MingCGSL022}
            & 30.91 & 94.61 & 37.59 & 92.57 & 44.69 & 89.77 & 57.77 & 86.11 & 42.74 & 90.77 \\
\hline
~ & \multicolumn{10}{c}{One-shot}\\
CoOp$\displaystyle _{MCM}$ \citep{DBLP:journals/ijcv/ZhouYLL22}
            & 43.38 & 91.26 & 38.53 & 91.95 & 46.68 & 89.09 & 50.64 & 87.83 & 44.81 & 90.03 \\
CoOp$\displaystyle _{GL}$ \citep{DBLP:journals/ijcv/ZhouYLL22}
            & 21.30 & 95.27 & 31.66 & 92.16 & 40.44 & 89.31 & 52.93 & 84.25 & 36.58 & 90.25 \\
LoCoOp$\displaystyle _{MCM}$ \citep{DBLP:journals/corr/abs-2306-01293}
            & 38.49 & 92.49 & 33.27 & 93.67 & 39.23 & 91.07 & 49.25 & 89.13 & 40.17 & 91.53 \\
LoCoOp$\displaystyle _{GL}$ \citep{DBLP:journals/corr/abs-2306-01293}
            & 24.61 & 94.89 & 25.62 & 94.59 & 34.00 & \textbf{92.12} & 49.86 & 87.49 & 33.52 & 92.14 \\
\rowcolor{gray!20}
Ours        & 15.46 & 97.16 & 39.15 & 92.12 & 41.35 & 90.86 & 32.07 & 93.12 & 32.01 & 93.32 \\
\hline
~ & \multicolumn{10}{c}{Four-shot}\\
CoOp$\displaystyle _{MCM}$ \citep{DBLP:journals/ijcv/ZhouYLL22}
            & 35.36 & 92.60 & 37.06 & 92.27 & 45.38 & 89.15 & 43.74 & 89.68 & 40.39 & 90.92 \\
CoOp$\displaystyle _{GL}$ \citep{DBLP:journals/ijcv/ZhouYLL22}
            & 18.95 & 95.52 & 29.58 & 92.90 & 38.72 & 89.64 & 48.03 & 85.87 & 33.82 & 90.98 \\
LoCoOp$\displaystyle _{MCM}$ \citep{DBLP:journals/corr/abs-2306-01293}
            & 29.45 & 93.93 & 33.06 & 93.24 & 41.13 & 90.32 & 44.15 & 90.54 & 36.95 & 92.01 \\
LoCoOp$\displaystyle _{GL}$ \citep{DBLP:journals/corr/abs-2306-01293}
            & 18.49 & 96.07 & 22.85 & 95.00 & \textbf{32.38} & 91.86 & 44.72 & 89.10 & 29.61 & 93.01 \\
\hline
\end{tabularx}
\end{table*}



==> tables/t_result_sun_statistical.tex <==
% \setlength{\abovecaptionskip}{3pt}
% \setlength{\belowcaptionskip}{-15pt}
\begin{table}[t]
% \vspace{1.5em}
\caption{OOD detection performance on SUN \citep{DBLP:conf/cvpr/XiaoHEOT10}.}
\label{result_sun_statistical}
\renewcommand{\arraystretch}{1.0}
\begin{tabularx}{0.47\textwidth}{
c|c|c
}

\hline
\multirow{2}{*}{SUN} & \multicolumn{2}{c}{ID scores} \\
\cmidrule(r){2-3}
~ & [0,0.5)& [0.5,1]\\
\hline
ID number &  13/200 & 132/200 \\
\hline
\end{tabularx}
% \vspace{-0.5em}
\end{table}
